Towards Real-time Traffic Sign and Traffic Light Detection on Embedded Systems

Recent work done on traffic sign and traffic light detection focus on improving detection accuracy in complex scenarios, yet many fail to deliver real-time performance, specifically with limited computational resources. In this work, we propose a simple deep learning based end-to-end detection framework, which effectively tackles challenges inherent to traffic sign and traffic light detection such as small size, large number of classes and complex road scenarios. We optimize the detection models using TensorRT and integrate with Robot Operating System to deploy on an Nvidia Jetson AGX Xavier as our embedded device. The overall system achieves a high inference speed of 63 frames per second, demonstrating the capability of our system to perform in real-time. Furthermore, we introduce CeyRo, which is the first ever large-scale traffic sign and traffic light detection dataset for the Sri Lankan context. Our dataset consists of 7984 total images with 10176 traffic sign and traffic light instances covering 70 traffic sign and 5 traffic light classes. The images have a high resolution of 1920 x 1080 and capture a wide range of challenging road scenarios with different weather and lighting conditions. Our work is publicly available at https://github.com/oshadajay/CeyRo.

==> figures/augmentation/fig2.tex <==
\begin{tikzpicture}

\setlength{\baselineskip}{5em}

\tikzstyle{bluebox}=[draw=cyan!20!black,fill=cyan!20]
\tikzstyle{greenbox}=[draw=green!20!black,fill=green!20]
\tikzstyle{orangebox}=[draw=yellow!20!black,fill=yellow!20]
\tikzstyle{magentabox}=[draw=magenta!20!black,fill=magenta!20]


\tikzstyle{labelnode}=[align=center, execute at begin node=\setlength{\baselineskip}{0.75em}]

\newcommand{\cube}[5][]
{
	\pgfmathsetmacro{\cubex}{(#2)}
	\pgfmathsetmacro{\cubey}{{#3}}
	\pgfmathsetmacro{\cubez}{{#4}}
	\draw[#5] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
	\draw[#5] (0,0,0) -- ++(0,0,-\cubez) -- ++(0,-\cubey,0) -- ++(0,0,\cubez) -- cycle;
	\draw[#5] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez) -- ++(\cubex,0,0) -- cycle;
}
\begin{scope}[xshift=0cm, yshift=0cm]
    \node[inner sep=0pt] (russell) at (0,0)
    {\includegraphics[height=.1\textwidth]{figures/augmentation/958bT_out.jpg}};
    \draw [-latex] (1.8, 0) -- ++(1.5, 0);

    
\end{scope}

\begin{scope}[xshift=4.8cm, yshift=0cm]
     \node[inner sep=0pt] (russell) at (0,0)
    {\includegraphics[height=.1\textwidth]{figures/augmentation/958bT_A1_out.jpg}};
  
\end{scope}



\end{tikzpicture}

==> figures/augmentation/fig3.tex <==
\begin{tikzpicture}

\setlength{\baselineskip}{5em}

\tikzstyle{bluebox}=[draw=cyan!20!black,fill=cyan!20]
\tikzstyle{greenbox}=[draw=green!20!black,fill=green!20]
\tikzstyle{orangebox}=[draw=yellow!20!black,fill=yellow!20]
\tikzstyle{magentabox}=[draw=magenta!20!black,fill=magenta!20]


\tikzstyle{labelnode}=[align=center, execute at begin node=\setlength{\baselineskip}{0.75em}]

\newcommand{\cube}[5][]
{
	\pgfmathsetmacro{\cubex}{(#2)}
	\pgfmathsetmacro{\cubey}{{#3}}
	\pgfmathsetmacro{\cubez}{{#4}}
	\draw[#5] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
	\draw[#5] (0,0,0) -- ++(0,0,-\cubez) -- ++(0,-\cubey,0) -- ++(0,0,\cubez) -- cycle;
	\draw[#5] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez) -- ++(\cubex,0,0) -- cycle;
}
\begin{scope}[xshift=0cm, yshift=0cm]
    \node[inner sep=0pt] (russell) at (0,0)
    {\includegraphics[height=.15\textwidth]{figures/augmentation/DWS-01_1183b_0_aug_flipr.jpg}};
    \draw [-latex] (2.2, 0) -- ++(1.5, 0);
    \node at (-.5, -1.5) [anchor=west] {\scriptsize DWS-01};

    
\end{scope}

\begin{scope}[xshift=5.8cm, yshift=0cm]
     \node[inner sep=0pt] (russell) at (0,0)
    {\scalebox{-1}[1]{\includegraphics[height=.15\textwidth]{figures/augmentation/DWS-01_1183b_0_aug_flipr.jpg}}};
    \node at (-.5, -1.5) [anchor=west] {\scriptsize DWS-02};
\end{scope}

\begin{scope}[xshift=0cm, yshift=3cm]
    \node[inner sep=0pt] (russell) at (0,0)
    {\includegraphics[height=.15\textwidth]{figures/augmentation/PHS-24_359d_0_aug_flipr.jpg}};
    \draw [-latex] (2.2, 0) -- ++(1.5, 0);
    \node at (-.5, -1.5) [anchor=west] {\scriptsize PHS-24};
    
\end{scope}

\begin{scope}[xshift=5.8cm, yshift=3cm]
     \node[inner sep=0pt] (russell) at (0,0)
    {\scalebox{-1}[1]{\includegraphics[height=.15\textwidth]{figures/augmentation/PHS-24_359d_0_aug_flipr.jpg}}};
    \node at (-.5, -1.5) [anchor=west] {\scriptsize PHS-24};
\end{scope}

\end{tikzpicture}

==> figures/classification_dataset/classification_dataset.tex <==
\begin{tikzpicture}

\setlength{\baselineskip}{5em}

\tikzstyle{bluebox}=[draw=cyan!20!black,fill=cyan!20]
\tikzstyle{greenbox}=[draw=green!20!black,fill=green!20]
\tikzstyle{orangebox}=[draw=yellow!20!black,fill=yellow!20]
\tikzstyle{magentabox}=[draw=magenta!20!black,fill=magenta!20]


\tikzstyle{labelnode}=[align=center, execute at begin node=\setlength{\baselineskip}{0.75em}]

\newcommand{\cube}[5][]
{
	\pgfmathsetmacro{\cubex}{(#2)}
	\pgfmathsetmacro{\cubey}{{#3}}
	\pgfmathsetmacro{\cubez}{{#4}}
	\draw[#5] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,-\cubey,0) -- ++(\cubex,0,0) -- cycle;
	\draw[#5] (0,0,0) -- ++(0,0,-\cubez) -- ++(0,-\cubey,0) -- ++(0,0,\cubez) -- cycle;
	\draw[#5] (0,0,0) -- ++(-\cubex,0,0) -- ++(0,0,-\cubez) -- ++(\cubex,0,0) -- cycle;
}
\begin{scope}[xshift=0cm, yshift=0cm]
    \node[inner sep=0pt] (russell) at (0,0)
    {\includegraphics[height=.10\textwidth]{figures/classification_dataset/1188.jpg}};
    \draw [-latex] (1.7, 0) -- ++(1.4, 0);

    
\end{scope}

\begin{scope}[xshift=5cm, yshift=0cm]
     \node[inner sep=0pt] (russell) at (-1,0)
    {\includegraphics[height=.09\textwidth]{figures/classification_dataset/1188_0.jpg}};
   \node at (-1.6, -1) [anchor=west] {\scriptsize SLS-40};
\end{scope}

\begin{scope}[xshift=7.5cm, yshift=0cm]
     \node[inner sep=0pt] (russell) at (-1.8,0)
    {\includegraphics[height=.09\textwidth]{figures/classification_dataset/1188_1.jpg}};
    \node at (-2.3, -1) [anchor=west] {\scriptsize APR-12};
   
\end{scope}

\end{tikzpicture}
